PlaneRCNN: 3D Plane Detection and Reconstruction from a Single Image

This paper proposes a deep neural architecture, PlaneRCNN, that detects and reconstructs piecewise planar surfaces from a single RGB image. PlaneRCNN employs a variant of Mask R-CNN to detect planes with their plane parameters and segmentation masks. PlaneRCNN then jointly refines all the segmentation masks with a novel loss enforcing the consistency with a nearby view during training. The paper also presents a new benchmark with more fine-grained plane segmentations in the ground-truth, in which, PlaneRCNN outperforms existing state-of-the-art methods with significant margins in the plane detection, segmentation, and reconstruction metrics. PlaneRCNN makes an important step towards robust plane extraction, which would have an immediate impact on a wide range of applications including Robotics, Augmented Reality, and Virtual Reality.

==> sec_results_debug.tex <==
\section{Experimental results}
We have implemented our network in PyTorch. We use pre-trained Mask R-CNN~\cite{he2017mask} and initialize the segmentation refinement network with the existing model~\cite{he2015delving}. We train the network end-to-end on an NVIDIA TitanX GPU for 10 epochs with 100,000 randomly sampled images from training scenes in ScanNet. We use the same scale factor for all losses. For the detection network, we scale the image to $640 \times 480$ and pad zero values to get a $640 \times640$ input image. For the refinement network, we scale the image to $256 \times 192$ and align the detected instance masks with the image based on the predicted bounding boxes.

\begin{figure}[t]
	\centering
    \includegraphics[width=.99\linewidth]{figures/curves_horizontal.jpg}
\caption{Plane-wise accuracy against baselines. PlaneRCNN outperforms all the competing methods except when the depth threshold is very small and MWS-G can fit 3D planes extremely accurately by utilizing the ground-truth depth values.}
	\label{fig:curves}
\end{figure}


\subsection{Qualitative evaluations}
\label{sect:qualitative}
Fig.~\ref{fig:results} demonstrates our reconstructions results for ScanNet testing scenes. PlaneRCNN is able to recover planar surfaces even for small objects.
We include more examples in Appendix~\ref{appendix:results}.

Fig.~\ref{fig:cross_dataset} compares PlaneRCNN against two competing methods, PlaneNet~\cite{liu2018planenet} and PlaneRecover~\cite{yang2018recovering}, on a variety of scene types from unseen datasets (except the SYNTHIA dataset is used for training by PlaneRecover).
Note that PlaneRCNN and PlaneNet are trained on the ScanNet which contains indoor scenes, while PlaneRecover is trained on the SYNTHIA dataset (i.e., the 7th and 8th rows in the figure) which consist of synthetic outdoor scenes. 
The figure shows that PlaneRCNN is able to reconstruct most planes in varying scene types from unseen datasets regardless of their sizes, shapes, and textures.
In particular,
our results on the KITTI dataset are surprisingly better than PlaneRecover for planes close to the camera. In indoor scenes, our results are consistently better than both PlaneNet and PlaneRecover.
We include more examples in Appendix~\ref{appendix:results}.

\begin{figure*}[htb]
\begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width=\linewidth]{figures/scannet_12.jpg}
\caption{Piecewise planar reconstruction results by PlaneRCNN. From left to right: input image, plane segmentation, depthmap reconstruction, and 3D rendering of our depthmap (rendered from a new view with -0.4m and 0.3m translation along x-axis and z-axis respectively and $10^{\degree}$ rotation along both x-axis and z-axis).}
    \label{fig:results}
\end{minipage}

\hfill
\begin{minipage}[t]{0.48\textwidth}
    \includegraphics[width=\linewidth]{figures/cross_dataset_labeled.jpg}
\caption{Plane segmentation results on unseen datasets without fine-tuning. From left to right: input image, PlaneNet~\cite{liu2018planenet} results, PlaneRecover~\cite{yang2018recovering} results, and ours. From top to the bottom, we show two examples from each dataset in the order of NYUv2~\cite{silberman2012indoor}, 7-scenes~\cite{shotton2013scene}, KITTI~\cite{geiger2013vision}, SYNTHIA~\cite{ros2016synthia}, Tank and Temple~\cite{knapitsch2017tanks}, and PhotoPopup~\cite{hoiem2005automatic}.
}
	\label{fig:cross_dataset}
\end{minipage}
\end{figure*}


\subsection{Plane reconstruction accuracy}
\label{sect:reconstruction}
Following PlaneNet~\cite{liu2018planenet}, we evaluate plane detection accuracy by measuring the plane recall with a fixed Intersection over Union (IOU) threshold $0.5$ and a varying depth error threshold (from $0$ to $1m$ with an increment of $0.05m$).
The accuracy is measured inside the overlapping regions between the ground-truth and inferred planes. Besides PlaneNet, we compare against Manhattan World Stereo (MWS)~\cite{furukawa2009manhattan}, which is the most competitive traditional MRF-based approach as demonstrated in prior evaluations~\cite{liu2018planenet}. 
MWS requires a 3D point cloud as an input, and we either use the point cloud from the ground-truth 3D planes (MWS-G) or the point cloud inferred by our depthmap estimation module in the plane detection network (MWS). 

PlaneRecover~\cite{yang2018recovering} was originally trained with the assumption of at most 5 planes in an image. We find it difficult to train PlaneRecover successfully for cluttered indoor scenes by simply increasing the threshold.
We believe that PlaneNet, which is explicitly trained on ScanNet, serves as a stronger competitor for the evaluation.

As demonstrated in \fig{fig:curves}, PlaneRCNN significantly outperforms all other methods,
except when the depth threshold is small and MWS-G can fit planes extremely accurately with the ground-truth depth values.

Nonetheless, even with ground-truth depth information, MWS-G fails in extracting planar regions robustly, leading to lower recalls in general.
%, making their detection recall lower in general. 
Our results are superior also qualitatively as shown 
%Qualitatively, our method is able to segment planar regions more accurately as shown
in~\fig{fig:comparison}.

\begin{figure*}
	\centering
	\newlength\exlen
    \setlength\exlen{\linewidth}
    \includegraphics[width=\linewidth]{figures/comparison_4.jpg}
\vspace{2pt}
\caption{Plane segmentation comparisons.
%gmentation results generated by different methods.
From left to right: input image, MWS~\cite{furukawa2009manhattan} with inferred depths, MWS~\cite{furukawa2009manhattan} with ground-truth depths, PlaneNet~\cite{liu2018planenet}, Ours, and ground-truth.}
	\label{fig:comparison}
	\vspace{3pt}
\end{figure*}

\subsection{Geometric accuracy}
\label{sect:geometry}
We propose a new metric in evaluating the quality of piecewise planar surface reconstruction by mixing the inferred depthmaps and the ground-truth plane segmentations. More precisely, we first generate a depthmap from our reconstruction by following the process in the warping loss evaluation (Sec.~\ref{sec:two-view-consistency}).
Next, for every ground-truth planar segment, we convert depth values in the reconstructed depthmap to 3D points, fit a 3D plane by SVD, and normalize the plane coefficients to make the normal component into a unit vector.
Finally, we compute the mean and the area-weighted mean of the parameter differences to serve as the evaluation metrics. Besides the plane parameter metrics, we also consider depthmap metrics commonly used in the literature~\cite{eigen2015predicting}. We evaluate over the NYU dataset~\cite{silberman2012indoor} for a fair comparison.
Table~\ref{tbl:comparison} shows that, with more flexible detection network, PlaneRCNN generalizes much better without fine-tuning. PlaneRCNN also outperforms PlaneNet~\cite{liu2018planenet} in every metric after fine-tuning using the ground-truth depths from the NYU dataset.

\begin{table}[h]
\caption{Geometric accuracy comparison over the NYUv2 dataset.
%\khnote{We need to discuss about DORN and CCRF and what is the important point of comparison over pure depth estimation today..} \khnote{Also unify the bold and color text: i.e., only bold or color for the best results..}
}
\label{tbl:comparison}
  \centering
  \begin{tabular}{l|c|c}
    \toprule
  Method & PlaneNet~\cite{liu2018planenet} & Ours \\
  \midrule
  \multicolumn{3}{c}{w/o fine-tuning} \\
  \midrule
  Rel & 0.220 & \textbf{0.164} \\
  $log_{10}$ & 0.114 & \textbf{0.077} \\
  $RMSE$ & 0.858 & \textbf{0.644} \\
  Param. & 0.939 & \textbf{0.776} \\
  Param. (weighted) & 0.771 & \textbf{0.641} \\
 \midrule
  \multicolumn{3}{c}{w/ fine-tuning} \\
  \midrule
  Rel & 0.129 & \textbf{0.124} \\
  $log_{10}$ & 0.079 & \textbf{0.073} \\
  $RMSE$ & 0.397 & \textbf{0.395} \\
  Param. & 0.713 & \textbf{0.642} \\
  Param. (weighted) & 0.532 & \textbf{0.505} \\
  \bottomrule
  \end{tabular}
\vspace{-5pt}
\end{table}

\subsection{Ablation studies}
\label{sect:ablation}
PlaneRCNN adds the following components to the Mask R-CNN~\cite{he2017mask} backbone: 1) the pixel-wise depth estimation network;
%to make plane parameters invariant to a location,
2) the anchor-based plane normal regression;
%representation for plane normal prediction,
3) the warping loss module; and 4)
%between two views during training, and 4) 
the segmentation refinement network.
%a refinement network to optimize plane segmentation globally.
%We add several components upon Mask R-CNN~\cite{he2017mask} backbone for our specific tasks. To be specific, we have
%
To evaluate the contribution of each component, we measure performance changes while adding the components one by one.
%we evaluate how plane detection performance changes by adding one component at each time.
%
Following~\cite{yang2018recovering}, we evaluate the plane segmentation quality by three clustering metrics: variation of information (VOI), Rand index (RI), and segmentation covering (SC). To further assess the geometric accuracy, we compute the average precision (AP) with IOU threshold $0.5$ and three different depth error thresholds $[0.4m, 0.6m, 0.9m]$. A larger value means higher quality for all the metrics except for VOI.
%The larger values 
%Except VOI which is the lower the better, all other metrics are the higher the better.

\tbl{tbl:ablation} shows that all the components have a positive contribution to the final performance.
%Disentangling plane parameter prediction into separate prediction of pixel-wise depth and plane normal lead to a large improvement on geometry accuracy reflected by average precision. The anchor-based normal prediction further improves geometry predictions.
\fig{fig:ablation} further highlights the contributions of the warping loss module and the segmentation refinement network qualitatively.
%qualitatively 
%To better understand the contributions of the warping loss module and the segmentation refinement network, 
%contribute to the final performance, we highlight the effect of each component in~\fig{fig:ablation}.
The first example shows that the segmentation refinement network fills in gaps between adjacent planar regions, while
%Note that there is still possible gaps in 3D space due to the imperfect geometry prediction but the segmentation refinement network alleviate the problem to a large extent.
the second example shows that the warping loss module improves reconstruction accuracy with the help from the second view.
%yields locally coherent reconstructions. \yfnote{I couldn't really understand "locally coherent". More clarification?}

\begin{table*}[h]
\caption{Ablation studies on the contributions of the four components in PlaneRCNN. Plane segmentation and detection metrics are calculated over the ScanNet dataset. PlaneNet represents the competing state-of-the-art.\\
}
\vspace{2pt}
\label{tbl:ablation}
  \centering
  \begin{tabular}{l|ccc|ccc}
    \toprule
  & \multicolumn{3}{c|}{Plane segmentation metrics} & \multicolumn{3}{c}{Plane detection metrics} \\
  \midrule
Method & VOI $\downarrow$ & RI & SC & AP$^{0.4m}$ & AP$^{0.6m}$ & AP$^{0.9m}$ \\
\midrule
PlaneNet & 2.142 & 0.797 & 0.692 & 0.156 & 0.178 & 0.182 \\
\midrule
Ours (basic) & 2.113 & 0.851 & 0.719 & 0.269 & 0.329 & 0.355 \\
Ours (depth) & 2.041 & 0.856 & 0.752 & 0.352 & 0.376 & 0.386 \\
Ours (depth + anch.) & 2.021 & 0.855 & 0.761 & 0.352 & 0.378 & 0.392 \\
Ours (depth + anch. + warp.) & 1.990 & 0.855 & 0.766 & \textbf{0.365} & 0.384 & 0.401 \\
\midrule
Ours (depth + anch. + warp. + refine.) & \textbf{1.809} & \textbf{0.880} & \textbf{0.810} & \textbf{0.365} & \textbf{0.386} & \textbf{0.405} \\
  \bottomrule
  \end{tabular}
\vspace{2pt}
\end{table*}


\begin{figure}[t]
	\centering
    \includegraphics[width=\linewidth]{figures/ablation.jpg}
\caption{Effects of the segmentation refinement network and the warping loss module.
%Qualitative evaluations for refinement and warping. 
Top: the refinement network narrows the gap between adjacent planes. Bottom: the warping loss helps
to correct erroneous plane geometries using the second view.}
%penalizes mistakes which causes erroneous geometries in the neighbor view.}
	\label{fig:ablation}
	\vspace{3pt}
\end{figure}


\subsection{Occlusion reasoning}
\label{sect:occlusion}
%\yfnote{Can we split into multiple paragraphs?}
%Representing the scene with planes provide more intuitive analysis on the 3D structure. 
A simple modification allows PlaneRCNN to infer occluded/invisible surfaces and reconstruct layered depthmap models. We add one more mask prediction module to PlaneRCNN to infer the complete mask for each plane instance.

The key challenge for training the network with occlusion reasoning is to generate ground-truth complete mask for supervision. In our original process, we fit planes to aligned 3D scans to obtain ground-truth 3D planar surfaces, then rasterize the planes to an image with a depth testing. We remove the depth testing and generate a ``complete mask" for each plane. Besides disabling depth checking, we further complete the mask for layout structures based on the fact that layout planes are behind other geometries. First, we collect all planes which have layout labels (e.g., \textit{wall} and \textit{floor}), and compute the convexity and concavity between two planes in 3D space. Then for each combination of these planes, we compute the corresponding complete depthmap by using the greater depth value for two convex planes and using the smaller value for two concave ones. A complete depthmap is valid if $90\%$ of the complete depthmap is behind the visible depthmap (with $0.2m$ tolerance to handle noise). We pick the valid complete depthmap which has the most support from visible regions of layout planes.

\fig{fig:occlusion} shows the new view synthesis examples, in which the modified PlaneRCNN successfully infers occluded surfaces, for example, floor surfaces behind tables and chairs. Note that a depthmap is rendered as a depth mesh model (i.e., a collection of small triangles) in the figure. The layered depthmap representation enables new applications such as artifacts-free view synthesis, better scene completion, and object removal~\cite{liu2016layered,tulsiani2018layer}. This experiment demonstrates yet another flexibility and potential of the proposed PlaneRCNN architecture.

\begin{figure}[h]
	\centering
    \includegraphics[width=\linewidth]{figures/occlusion.jpg}
\caption{New view synthesis results with the layered depthmap models. A simple modification allows PlaneRCNN to also infer occluded surfaces and reconstruct layered depthmap models.
}
	\label{fig:occlusion}
\end{figure}

